A Distribution-Dependent Analysis of Meta-Learning

A key problem in the theory of meta-learning is to understand how the task distributions influence transfer risk, the expected error of a meta-learner on a new task drawn from the unknown task distribution. In this paper, focusing on fixed design linear regression with Gaussian noise and a Gaussian task (or parameter) distribution, we give distribution-dependent lower bounds on the transfer risk of any algorithm, while we also show that a novel, weighted version of the so-called biased regularized regression method is able to match these lower bounds up to a fixed constant factor. Notably, the weighting is derived from the covariance of the Gaussian task distribution. Altogether, our results provide a precise characterization of the difficulty of meta-learning in this Gaussian setting. While this problem setting may appear simple, we show that it is rich enough to unify the "parameter sharing" and "representation learning" streams of meta-learning; in particular, representation learning is obtained as the special case when the covariance matrix of the task distribution is unknown. For this case we propose to adopt the EM method, which is shown to enjoy efficient updates in our case. The paper is completed by an empirical study of EM. In particular, our experimental results show that the EM algorithm can attain the lower bound as the number of tasks grows, while the algorithm is also successful in competing with its alternatives when used in a representation learning context.

==> conclusions.tex <==
%
We proved the first instance-dependent universal lower bound on the transfer risk for meta-learning in the linear regression with fixed design.
Moreover, we demonstrated that a weighted form of a biased regularization enjoys upper bound on the risk matching the lower bound up to a multiplicative constant --- establishing instance-dependent optimality of a biased regularization, a popular tool in transfer learning literature.
Thus, our bounds \emph{characterize} meta-learning linear regression problems and reveal a fine-grained dependency on the task structure.
In particular, this characterization implies that learning of a regression function can happen much faster than in a single task learning, given a specific task structure.
%
A natural future direction for our work is a instance-dependent characterization in a more general setting, such as regression with random inputs, and going beyond linear setting, e.g.\ by studying meta-learning in nonparameteric regression.
Finally, we proposed an effective \ac{EM} procedure for task structure estimation. An interesting future problem is to understand the performance of \ac{EM} in our meta-learning setting theoretically.

==> related.tex <==
%!TEX root =  icml.tex
%
% Early generalization analysis in meta-learning~\citep{baxter2000model,maurer2005algorithmic} focused on bounds on the generalization gap in a instance-independent setting showcasing the interaction between the number of tasks, the sample size, and the capacity of the parameter class.
% Later on, the community started to pay attention to the instance-dependent setting where the generalization gap is also controlled by the quantities capturing task relatedness, such as $\tau^2$ or eigenvalues of $\bSigma$ featuring in this paper.
% To name a few, \cite{li2007bayesian,pentina2014pac,amit2018meta} gave a PAC-Bayesian analysis of the generalization gap while~\cite{kuzborskij2013stability} revisited an algorithmic stability analysis for the case of $n=2$.

% However, as pointed out earlier, the notion of generalization gap might fall short to fully explain learning abilities of algorithms and to compare them. To this end, the literature on meta-learning also considered the excess risk (the gap between the risk and the risk of the best-in-the-class): in particular, \cite{maurer2016benefit} proved upper bounds on the excess risk in multi-task and meta-learning scenarios when learning with dictionary representations.
% The rates in the same setting were recently improved by~\cite{du2020few} to $\gO(1/(n m) + 1/m)$ for excess risk in expectation.
% In this paper we try to address less studied topic of lower bounds on the excess risk in a instance-dependent setting.

In the recent years, meta-learning community dedicated considerable effort to the design and analysis of meta-learning algorithms able to learn in a sequential setting.
An early notable line of research here is meta-leaning for non-i.i.d.\ sequence of tasks investigated by~\cite{pentina2015lifelong,pentina2016lifelong}.
With the advent of the tremendous success of \ac{GD}-based meta-learning in deep neural networks~\citep{finn2017model}, the field focused largely on the design of \ac{GD}-type algorithms and their analysis, inspired by the online learning with individual
sequences~\citep{alquier2017regret,franceschi2018bilevel,finn2019online,fallah2020convergence}, and recently demonstrated optimality of such algorithms~\citep{balcan2019provable,saunshi2020sample}.
Although online meta-learning goes beyond the scope of this paper, we note that estimators studied in this paper can easily be extended to sequential setting through rank-one updates of matrix inverses.

Biased regularization revisited in this paper has been a topic of interest in transfer learning for a long time in applications~\citep{kienzle2006personalized,yang2007cross} and theory~\citep{ben2013domain,kuzborskij2016fast}.
To the best of our knowledge, in this paper we show the first result regarding optimality of the \emph{weighted} biased regularization.
%
Biased regularization and the regression model discussed in this paper can be naturally described from the Bayesian point of view~\citep{grant2018recasting}.
Indeed, it is well-known that ridge regression with regularization biased to $\balpha$ arises as \ac{MLE} of a regression model with Gaussian-distributed parameters centered at $\balpha$.
The Bayesian point of view has been, for a long time (see discussion by~\cite{baxter2000model}), a source of inspiration for design of transfer learning algorithms~\citep{tommasi2010safety,salakhutdinov2012one} and even recent interpretations of \ac{GD}-based techniques such as MAML~\citep{grant2018recasting}.
While algorithms discussed in this paper can be seen as Bayesian, \todoc{MLE? EM??} the analysis we follow is fully frequentist.

Several works investigated a principled way of setting the bias in biased regularization~\citep{du2017hypothesis,denevi2018learning,denevi2019learning,bai2020important}, such as by averaging parameter estimates of previously observed or held-out tasks~\citep{denevi2018learning}.
In this paper we propose an optimal setting of the bias in the considered regression problem based on \ac{MLE}, and demonstrate that in order to achieve optimality one has to use a \emph{weighted} biased regularization.


%Finally, very recently~\cite{lucas2020theoretical} established universal \emph{minimax} (that is by taking $\sup$ over task distributions) lower bounds for meta learning.
%In this paper we explore a rather different, \emph{instance-dependent} characterization of meta-learning which demands the dependence on task distributions.
%Beyond linear regression setting, no-free-lunch results in meta-learning and multi-task learning have also recently received attention in nonparametric prediction~\citep{hanneke2020nofreelunch}.









